Model-checking parametric lock-sharing systems against regular constraints

In parametric lock-sharing systems processes can spawn new processes to run in parallel, and can create new locks. The behavior of every process is given by a pushdown automaton. We consider infinite behaviors of such systems under strong process fairness condition. A result of a potentially infinite execution of a system is a limit configuration, that is a potentially infinite tree. The verification problem is to determine if a given system has a limit configuration satisfying a given regular property. This formulation of the problem encompasses verification of reachability as well as of many liveness properties. We show that this verification problem, while undecidable in general, is decidable for nested lock usage. We show Exptime-completeness of the verification problem. The main source of complexity is the number of parameters in the spawn operation. If the number of parameters is bounded, our algorithm works in Ptime for properties expressed by parity automata with a fixed number of ranks.

==> Figures/fig1.tex <==
\begin{tikzpicture}[node distance=1.8cm,auto,>= triangle
	45,scale=.6]
	\tikzstyle{initial}= [initial by arrow,initial text=,initial
	distance=.7cm, initial where= below]
	\tikzstyle{accepting}= [accepting by arrow,accepting text=,accepting
	distance=.7cm,accepting where =right]
	
	\node[state,initial] (es) at (0,0) {$\dashover{\es}$};
	\node[state] (1w) at (3.2,4) {$\dashover{\set{1}}$};
	\node[state] (1s) at (9,4) {$\fillover{\set{1}}$};
	\node[state] (2w) at (-3.2,4) {$\dashover{\set{2}}$};
	\node[state] (2s) at (-9,4) {$\fillover{\set{2}}$};
	\node[state] (12) at (0,8) {$\dashover{\set{1,2}}$};
	%	\node[state] (q11) [right of =q10] {11};
	%	\node[state] (q12) [right of =q11] {12};
	
	
	
	\path[->, bend left=20] 	
	(es) edge node[left] {$\get{t_2}$} (2w)
	(1s) edge node[below] {$\rel{t_1}$} (es)
	(1s) edge node[above right] {$\get{t_2}$} (12)
	(12) edge node {$\rel{t_2}$} (1s)
	;
	\path[->, bend right=20] 
	(es) edge node[right] {$\get{t_1}$} (1w)
	(2s) edge node[below] {$\rel{t_2}$} (es)
	(2s) edge node {$\get{t_1}$} (12)
	(12) edge node[above left] {$\rel{t_1}$} (2s);
	%	(q10) edge node {$\rel{s1}$} (q11)
	%	(q11) edge node {$\get{p}$} (q12)
	%	(q3) edge node {$\get{\bp}$} (q12)
	%	(q5) edge[bend right] node {$\get{\bp}$} (q12)
	\path[->]
	(2w) edge node[right] {$\get{t_1}$} (12)
	(2w) edge node {$\rel{t_2}$} (es)
	(1w) edge node[above left] {$\rel{t_1}$} (es)
	(1w) edge node[left] {$\get{t_2}$} (12)
	(es) edge [out=330, in=300, looseness=8] node {$\nop$} (es)
	(1w) edge [loop right] node {$\nop$} ()
	(1s) edge [loop above] node {$\nop$} ()
	(2w) edge [loop left] node {$\nop$} ()
	(2s) edge [loop above] node {$\nop$} ()
	(12) edge [loop above] node {$\nop$} ()
	
	;
\end{tikzpicture}

==> Figures/fig2.tex <==
\begin{tikzpicture}[node distance=1.8cm,auto,>= triangle
	45,scale=.6]
	\tikzstyle{initial}= [initial by arrow,initial text=,initial
	distance=.7cm, initial where= left]
	\tikzstyle{accepting}= [accepting by arrow,accepting text=,accepting
	distance=.7cm,accepting where =right]
	
	\node[state,initial, minimum size=15pt] (p1) at (0,0) {};
	\node[state, minimum size=15pt] (p2) at (3,0) {};
	
	\node[state,initial, minimum size=15pt] (p'1) at (6,0) {1};
	\node[state, minimum size=15pt] (p'2) at (9,0) {2};
	\node[state, minimum size=15pt] (p'3) at (12,0) {3};

	\node[state, minimum size=15pt, initial] (Ci1) at (0,-3) {};
	\node[state, minimum size=15pt] (Ci2) at (3,-3) {};
	\node[state, minimum size=15pt] (Ci3) at (6,-3) {};
	
	\node[state, minimum size=15pt, initial] (li1) at (0,-6) {};
	\node[state, minimum size=15pt] (li2) at (3,-6) {};
	\node[state, minimum size=15pt] (li3) at (6,-6) {};
	
	
	\node[state, minimum size=15pt, initial] (xi1) at (9,-4) {};
	\node[state, minimum size=15pt] (xi2) at (12,-3) {};
	\node[state, minimum size=15pt] (xi3) at (12,-5) {};
	
	\node (x) at (8.4,-5) {\Large\textbf{$p^x_k$}};
	\node (l) at (-0.6,-7) {\Large\textbf{$p^\ell_{i,j}$}};
	\node (C) at (-0.6,-4) {\Large\textbf{$p^C_i$}};
	\node (p') at (5.4,-1) {\Large\textbf{$p'$}};
	\node (p) at (-0.6,-1) {\Large\textbf{$p$}};
	
	\path[->] 	
	(p1) edge node[above] {$\get{t}$} (p2)
	(Ci1) edge node[above] {$\get{t(C_i)}$} (Ci2)
	(Ci2) edge node[above] {$\get{t'}$} (Ci3) 
	
	
	(xi1) edge node[below] {$\get{t(x_k)}$} (xi3)
	(xi1) edge node[above=10pt] {$\get{t(\neg x_k)}$} (xi2)
	;
	\path[->, bend right=20] 
	(p'1) edge node[below] {$\get{t}$} (p'2)
	(p'2) edge node[above] {$\rel{t}$} (p'1)
	(p'2) edge node[below] {$\get{t'}$} (p'3)
	(p'3) edge node[above] {$\rel{t'}$} (p'2)
	
	(li1) edge node[below] {$\get{t(C_i)}$} (li2)
	(li2) edge node[above] {$\rel{t(C_i)}$} (li1)
	(li2) edge node[below] {$\get{t(\ell_{i,j})}$} (li3)
	(li3) edge node[above] {$\rel{t(\ell_{i,j})}$} (li2)
	%	(q10) edge node {$\rel{s1}$} (q11)
	%	(q11) edge node {$\get{p}$} (q12)
	%	(q3) edge node {$\get{\bp}$} (q12)
	%	(q5) edge[bend right] node {$\get{\bp}$} (q12)
	;
	\path[->, loop above] (p2) edge (p2);
\end{tikzpicture}

==> Figures/fig3.tex <==
\begin{tikzpicture}[node distance=1.8cm,auto,>= triangle
	45,scale=.6]
	\tikzstyle{initial}= [initial by arrow,initial text=,initial
	distance=.7cm, initial where= left]
	\tikzstyle{accepting}= [accepting by arrow,accepting text=,accepting
	distance=.7cm,accepting where =right]
	
	\node[state, minimum size=15pt,initial] (s1) at (0,0) {1};
	\node[state, minimum size=15pt] (s2) at (3,0) {2};
	\node[state, minimum size=15pt] (s3) at (6,0) {3};
	\node[state, minimum size=15pt] (s4) at (10,-1) {4};
	\node[state, minimum size=15pt] (s5) at (14,0) {5};
	\node[state, minimum size=15pt] (s6) at (10,1) {6};
	
	\path[->] 	
	(s1) edge node[above] {$\get{t_1}$} (s2)
	(s2) edge node[above] {$\get{t_2}$} (s3)
	;
	\path[->, bend right=20] 
	(s3) edge node[below left] {$\rel{t_1}$} (s4)
	(s4) edge node[below right] {$\get{t_1}$} (s5)
	(s5) edge node[above right] {$\rel{t_2}$} (s6)
	(s6) edge node[above left] {$\get{t_2}$} (s3)
	;
\end{tikzpicture}

==> Figures/fig5.tex <==
\begin{tikzpicture}[node distance=1.8cm,auto,>= triangle
	45,scale=.6]
	\tikzstyle{initial}= [initial by arrow,initial text=,initial
	distance=.7cm, initial where= left]
	\tikzstyle{accepting}= [accepting by arrow,accepting text=,accepting
	distance=.7cm,accepting where =right]
	
	\node[ minimum size=15pt] (G0) at (0,0) {$\G x$};
	\node[minimum size=15pt] (G1) at (-1,-2) {$\G x$};
	\node[minimum size=15pt] (G2) at (1,-2) {$\GN \s(x)$};
	
	\node[minimum size=15pt] (G3) at (5,0) {$\G x$};
	\node[minimum size=15pt] (G4) at (4,-2) {$\G x$};
	
	\node[ minimum size=15pt] (GN0) at (10,0) {$\GN x$};
	\node[minimum size=15pt] (GN1) at (9,-2) {$\GN x$};
	\node[minimum size=15pt] (GN2) at (11,-1.7) {$\GN \s(x)$};
	
	\node[minimum size=15pt] (GN3) at (15,0) {$\GN x$};
	\node[minimum size=15pt] (GN4) at (14,-1.7) {$\GN x$};
	
	\node[ minimum size=15pt] (EFG0) at (0,-3.5) {$\EFG x$};
	\node[minimum size=15pt] (EFG1) at (-1,-5.5) {$\EFG x$};
	\node[minimum size=15pt] (EFG2) at (1,-5.2) {$\AFGN \s(x)$};
	
	\node[ minimum size=15pt] (EFG3) at (5,-3.5) {$\EFG x$};
	\node[minimum size=15pt] (EFG4) at (4,-5.5) {$\AFGN x$};
	\node[minimum size=15pt] (EFG5) at (6,-5.2) {$\EFG \s(x)$};
	
	\node[minimum size=15pt] (EFG6) at (10,-3.5) {$\EFG x$};
	\node[minimum size=15pt] (EFG7) at (9,-5.5) {$\G x$};
	
	\node[minimum size=15pt] (EFG8) at (15,-3.5) {$\EFG x$};
	\node[minimum size=15pt] (EFG9) at (14,-5.2) {$\EFG x$};
	
	\node[ minimum size=15pt] (AGF0) at (0,-7) {$\AGFN x$};
	\node[minimum size=15pt] (AGF1) at (-1,-9) {$\AGFN x$};
	\node[minimum size=15pt] (AGF2) at (1,-8.7) {$\AGFN \s(x)$};
	
	\node[minimum size=15pt] (AGF3) at (5,-7) {$\AGFN x$};
	\node[minimum size=15pt] (AGF4) at (4,-9) {$\AGFN x$};
	
	\node[ minimum size=15pt] (AFG0) at (10,-7) {$\AFGN x$};
	\node[minimum size=15pt] (AFG1) at (9,-9) {$\AFGN x$};
	\node[minimum size=15pt] (AFG2) at (11,-8.7) {$\AFGN \s(x)$};
	
	\node[ minimum size=15pt] (AFG3) at (15,-7) {$\AFGN x$};
	\node[minimum size=15pt] (AFG4) at (14,-9) {$\AFGN x$};
	\node[minimum size=15pt] (AFG5) at (16,-8.7) {$\GN \s(x)$};
	
	\node[ minimum size=15pt] (AFG6) at (0,-10.5) {$\AFGN x$};
	\node[minimum size=15pt] (AFG7) at (-1,-12.5) {$\GN x$};
	\node[minimum size=15pt] (AFG8) at (1,-12.2) {$\AFGN \s(x)$};
	
	\node[ minimum size=15pt] (AFG9) at (5,-10.5) {$\AFGN x$};
	\node[minimum size=15pt] (AFG10) at (4,-12.5) {$\GN x$};
	\node[minimum size=15pt] (AFG11) at (6,-12.2) {$\GN \s(x)$};
	
	
	\node[minimum size=15pt] (AFG12) at (10,-10.5) {$\AFGN x$};
	\node[minimum size=15pt] (AFG13) at (9,-12.5) {$\AFGN x$};
	
	\node[minimum size=15pt] (AFG14) at (15,-10.5) {$\AFGN x$};
	\node[minimum size=15pt] (AFG15) at (14,-12.5) {$\GN x$};
	
	\path[-] 
	(G0) edge (G1)
	(G0) edge (G2)
	(G3) edge (G4)
	
	(GN0) edge (GN1)
	(GN0) edge (GN2)
	(GN3) edge (GN4)
	
	(EFG0) edge (EFG1)
	(EFG0) edge (EFG2)
	(EFG3) edge (EFG4)
	(EFG3) edge (EFG5)
	(EFG6) edge (EFG7)
	(EFG8) edge (EFG9)
	
	(AGF0) edge (AGF1)
	(AGF0) edge (AGF2)
	(AGF3) edge (AGF4)
	
	(AFG0) edge (AFG1)
	(AFG0) edge (AFG2)
	(AFG3) edge (AFG4)
	(AFG3) edge (AFG5)
	(AFG6) edge (AFG7)
	(AFG6) edge (AFG8)
	(AFG9) edge (AFG10)
	(AFG9) edge (AFG11)
	(AFG12) edge (AFG13)
	(AFG14) edge (AFG15);
\end{tikzpicture}

==> Proof-limit-local.tex <==
\begin{lemma}\label{lem:limitlocal}
	Suppose that $\tree$ satisfies the first three conditions of
	Lemma~\ref{lem:limit}.
	
	The relation $\prec_H$ is acyclic
	if and only if
	there a family of strict total orders 
	$<_\n$ over a subset of variables from $\Var{\n}$ with
	$\vallabel(\n)(x) \in H(\tree)$ such that:
	\begin{description}
		\item[F4.1] $x$ is ordered by $<_\n$ iff $L(\n)(x)\in H(\t)$.
		\item[F4.2] if $x <_\nu x'$, $\nu'$ is a child of
		$\nu$, and $y, y' \in \Var{\nu'}$ are such that $x \sim y$ and $x' \sim
		y'$ then $y <_{\nu'} y'$. 
		\item[F4.3]  if $x,x'\in  \Var{\nu}$ and $\vallabel(\n)(x) \prec_H \vallabel(\n)(x')$ then $x <_\n x'$.
	\end{description}
\end{lemma} 

\begin{proof}
	For the left-to-right direction we fix a strict total order $<$ on
	$H(\tree)$ that is compatible with $\prec_H$ (for instance the
	strict order $<$ defined in the proof of Lemma~\ref{lem:limit}).
	Then we order the variables $x \in \Var{\nu}$ with
	$\vallabel(\n)(x) \in H(\tree)$ according to $<$.
	The three conditions of the lemma then follow directly.
	
	For the converse we define $\prec$ on $H(\tree)$ by
	$\ell \prec \ell'$ if for some node $\n$ with variables $x\not=
	x'$ such that $\vallabel(\n)(x)=\ell$ and
	$\vallabel(\n)(x')=\ell'$ we have $x <_\n x'$.

	
	We start by showing that $\prec$ is acyclic.
	Assume by contradiction that $\ell_0\prec \ell_1 \cdots \prec
	\ell_k \prec \ell_0$ is a cycle of  minimal length, so
	the locks $\ell_i \in H(\tree)$ are all distinct.
	We use indices modulo $k+1$, so $k+1\equiv 0$.
	Note that $k>1$ because of condition F4.2.
	
	By assumption, the "scopes" of $\ell_i$ and $\ell_{i+1}$
	intersect, for every $i$.
	Since "scopes" are subtrees of $\tree$ (Remark~\ref{rem:scope})
	this means that two scopes that intersect have roots that are
	ordered by the ancestor relation in $\tree$.
	
	Assume first that $k>2$.
	Let $i$ be such that the depth of the root of the  "scope" of
	$\ell_i$ is maximal.
	So the roots of the "scopes" of $\ell_{i-1}$ and  $\ell_{i+1}$ are
	ancestors of the root $\n$ of the "scope" of $\ell_i$.
	In the "scope" of $\ell_i$ there exist nodes that belong to the
	"scope" of $\ell_{i-1}$ and of $\ell_{i+1}$, respectively.
	This means that $\n$ is in the scope of $\ell_{i-1},\ell_i$ and
	$\ell_{i+1}$.
	So the "scopes" of $\ell_{i-1}$ and $\ell_{i+1}$ intersect, and we
	have either $\ell_{i-1} <_\n \ell_{i+1}$ or $\ell_{i+1} <_\n
	\ell_{i-1}$.
	Thus we get from the definition of $\prec$ either
	$\ell_{i-1} \prec \ell_{i+1}$ or $\ell_{i+1} \prec    \ell_{i-1}$. 
	In both cases the cycle $\ell_0\prec \ell_1 \cdots \prec 
	\ell_k \prec \ell_0$ is not minimal, a contradiction.
	
	It remains to consider the case $\ell_0 \prec \ell_1 \prec \ell_2
	\prec \ell_0$.
	With a similar argument as before there exists a node $\n$ which is in
	the "scope" of all of $\ell_0,\ell_1,\ell_2$, so this node gives a
	total order on these locks and there cannot exist a cycle. 
	
	We now show that $\bef$ is acyclic as well.
	
	Like before, suppose there exists a cycle of distinct nodes $\ell_0 \bef \ell_1 \bef \cdots \bef \ell_k \bef \ell_{k+1} = \ell_0$ with $k > 0$. We consider such a cycle of minimal size. Hence for all $0\leq i \leq k$, $\ell_i$ is comparable with $\ell_{i-1}, \ell_i, \ell_{i+1}$ and incomparable with all the other $\ell_j$ (as otherwise we would obtain a shorter cycle).
	
	Given $\ell, \ell' \in TL$ such that $\ell \bef \ell'$, let $\nu$ be the node with an "unmatched" get of $\ell$. By condition~F3, this node is unique.
	
	This node has a descendant $\nu'$ with an operation on $\ell'$. There are two possibilities, one is that $\subtree(\ell)$ and $\subtree(\ell')$ intersect, in which case by condition~F4.3 we have $\ell \prec \ell'$.
	The other possibility is that the two subtrees do not intersect, in which case the root of $\subtree(\ell')$ is strictly below the "unmatched" get of $\ell$. 
	
	As $\prec$ is acyclic, there exist $i$ such that $\subtree(\ell_{i-1})$ and $\subtree(\ell_{i})$ are disjoint, hence all nodes of $\subtree(\ell_{i})$ are below the "unmatched" get of $\ell_{i-1}$. In particular the "unmatched" get of $\ell_{i-1}$ is an ancestor of the "unmatched" get of $\ell_{i}$. As a result, by the definition of $\bef$, $\ell_{i-1} \bef \ell_{i+1}$.
	
	If $k \geq 2$ then $\ell_0 \bef \ell_1 \bef \cdots \bef \ell_{i-1} \bef \ell_{i} \bef \cdots \bef \ell_{k+1} = \ell_0$ is a shorter cycle of distinct nodes, yielding a contradiction as we assumed the previous one to be minimal.
	
	If $k = 1$ then we have a contradiction as all nodes of $\subtree(\ell_{i})$ are below the "unmatched" get of $\ell_{i-1}$, in order to have $\ell_i \prec \ell_{i-1}$, we need a $\get{}$ on $\ell_{i-1}$ to happen in a descendant of its own "unmatched" get, which is impossible as then we would have $\ell_{i-1} \bef \ell_{i-1}$ and thus $\ell_{i-1} \prec \ell_{i-1}$ by condition F4.3, contradicting the acyclicity of $\prec$. 
	
	As a result, the relation $\bef$ is acyclic.
\end{proof}

==> Pspaceproof.tex <==
\section{Proof of Proposition~\ref{prop:PSPACE-LSS}}
\label{app:pspace-lss}

\PSPACELSS*

	The \PSPACE~upper bound is easy to obtain: It suffices to guess a state $s_p$ in each $\aut_p$ and $s'_p$ in each $\objaut{p}$, and then guess a sequence of letters in $\S$ while keeping track of the states reached by that sequence in the $\aut_p$ and $\objaut{p}$. 
	
	If we reach a configuration with each $\aut_p$ in state $s_p$ and each $\objaut{p}$ in $s'_p$, we start memorising the set of visited states in each $\objaut{p}$. 
	If we reach that configuration again, we stop and accept if and only if the set of visited states in the $\objaut{p}$ satisfies $\phi$.
	This comes down to guessing an ultimately periodic run in the global system and checking that it satisfies the objective.
	
	The difficulty is to obtain the \PSPACE-hardness with a fixed number of locks per process. To do so we reduce the emptiness problem for the intersection of a set of deterministic automata. 
	
	Without loss of generality we will assume that there are at least two automata, that they are all over alphabet $\set{0,1}$, and that their languages are all included in $11(00+01)^*$: we can always apply a small transformation to each automaton so that, if its language was $\mathcal{L}$, it becomes $11 h(\mathcal{L})$ with $h$ the morphism mapping $0$ to $00$ and $1$ to $01$. The intersection of those languages is empty if and only if the intersection of the original languages was empty.
	
	Let $\aut_1, \cdots, \aut_n$ (with $n \geq 2$) be automata, with, for each $1 \leq i \leq n$, $\aut_i = (S_i, \set{0,1}, \delta_i, init_i, F_i)$.
	We construct a "sound" "exclusive" "LSS" $\tss$ as follows:
	
	For each $1 \leq i \leq n$ we have a process $p_i$ which is in charge of simulating $\aut_i$.	
	The set of locks is $T = \set{0_i, 1_i, key_i \mid 1 \leq i \leq n}$.
	For all $i$, $p_i$ accesses locks $0_i, 1_i, key_i$, as well as $0_{i+1}, 1_{i+1}, key_{i+1}$ if $i \leq n-1$ and $0_{1}, 1_1$ if $i =n$. Thus a process uses at most 6 locks in total.
	
	For all $1 \leq i \leq n$ and $t$ accessed by $p_i$, we have two actions $\get{t}^i$ and $\rel{t}^i$, with which $p_i$ acquires and releases lock $t$, as well as actions $\nop^i$ and $end^i$ with no effect on locks.
	
	In the proof the following local sequences will be important:
	
	\[\send(0) = \rel{0_n}^n \get{0_{0}}^n \rel{1_n}^n \get{1_0}^n \rel{0_{0}}^n \get{0_n}^n \rel{1_{0}}^n \get{1_n}^n\]
	
	\[\rec_i(0) = \nop^i \get{0_{i+1}}^i \rel{0_{i}}^i \get{1_{i+1}}^i \rel{1_{i}}^i \get{0_{i}}^i \rel{0_{i+1}}^i \get{1_{i}}^i \rel{1_{i+1}}^i\]
	
	
	$\send(1)$ and $\rec_i(1)$ are defined analogously, by replacing $0$ by $1$ and $1$ by $0$ everywhere.
	
	The following global sequences will be useful as well:
	
	\[ \acqs(0) = \get{0_{n}}^{n-1}\rel{0_{n-1}}^{n-1} \cdots  \get{0_{1}}^{1}\rel{0_{0}}^{1}\]
	
	\[ \rels(0) = \get{0_{0}}^{1}\rel{0_{1}}^{1} \cdots  \get{0_{n-1}}^{n-1}\rel{0_{n}}^{n-1}\]
	
	\[ \NOP = \nop^{1} \cdots  \nop^{n-1}\]
	
	$\acqs(1)$ and $\rels(1)$ are defined analogously, by replacing $0$ by $1$ and $1$ by $0$ everywhere.	
	
	The transition system of each process $p_i$ is designed as follows: 
	We start with $\aut_i$, and we replace every transition labelled $0$ with a sequence of transitions labelled by actions of $\send(0)$ if $i=n$, and $\rec_i(0)$ if $1 \leq i \leq n-1$ (there is at least one such $i$ as $n \geq 2$).
	
	Furthermore we add a few transitions so that each $p_i$ with $i \leq n-1$ executes $\start_i = \get{key_{i+1}}^i \get{0_i}^i \get{1_i}^i  \get{key_i}^i \rel{key_{i+1}}^i$ before entering the initial state of $\aut_i$.
	If $i=n$ that sequence is $\start_n = \get{a_n}^n \get{b_n}^n \get{key_n}^n$.
	We also add a transition reading $end^i$ from all states of $F_i$ to a state $stop_i$ with no outgoing transition.
	
	The objective is that the action $end^i$ is executed for all $1 \leq i \leq n$.
	
	One direction is easy.
	Say there is a word $u = b_1 b_2 \cdots b_m$ in the intersection of the languages of the $\aut_i$. Then we start by executing all $\start_i$ sequences for all $i$ in increasing order, and then, for each $1 \leq j \leq m$ (in increasing order), we execute the sequence of operations 
	
	
	\begin{align*}
		seq(b_j) = &\rel{(b_j)_n}^n \NOP~\acqs(b_j) \get{(b_j)_0}^n \rel{(1-b_j)_n}^n\\ &\acqs(1-b_j) \get{(1-b_j)_0}^n \rel{(b_j)_0}^n \rels(b_j)\\ &\get{(b_j)_n}^n\rel{(1-b_j)_0}^n \rels(1-b_j) \get{(1-b_j)_n}^n 
	\end{align*}
	
	
	This run projects on $p_i$ as $\start_i \rec_i(b_1) \rec_i(b_2) \cdots \rec_(b_m)$ if $i\leq n-1$ and $\start_i \send(b_1) \send(b_2) \cdots \send(b_m)$ if $i=n$. As $u$ is in the language of $\aut_i$, $p_i$ can execute this run locally.
	It can be easily checked that all operations in that run are valid in the current configuration, hence this sequence can be executed.
	
	As $u$ is accepted by all $\aut_i$, after executing the sequence above each process $p_i$ ends up in a state of $F_i$, and thus they can all execute $end^i$ one after the other.
	
	Conversely, suppose there is some run $\run$ whose local projection $\run|_p$ on each process $p$ is ends with $end^i$.
	Each $\run|_{p_i}$ must start with the execution of $\start_i$.
	
	We prove the following lemma:
	
	\begin{lemma}
		For all $j \in \nats$, let $\run_j$ be the shortest prefix of $\run$ whose projection on $p_n$ is $\start_n \send(b_1) \cdots \send(b_j)$. 
		Then the projection of $\run_j$ on every other $p_i$ has $\rec_i(b_1) \cdots \rec_i(b_j)$ as a suffix.
	\end{lemma}

	\begin{proof}
		We prove this by induction on $j$.
		For $j=0$ it is trivial.
		Let $j \in \nats$, suppose the claim is true for $j$, we show it for $j+1$.
		
		First of all note that for all $i \geq 1$, if $p_i$ has finished executing $\start_i$ then it holds $k_i$ and will never release it, hence $p_{i-1}$ either has executed $\start_{i-1}$ in full or has not begun executing it. In the second case, $p_{i-1}$ will never be able to advance, which is impossible as $\run|_p$ is not empty. As a result, after $p_n$ has executed $\start_n$, all other $p_i$ must have executed $\start_i$.
		
		Another important remark is that after executing $\start_i$, all $p_i$ alternate between a $\get{}$ and a $\rel{}$ no matter which local run they execute. While $p_n$ starts with a $\rel{}$, all other processes start with a $\get{}$. Therefore $p_n$ always holds either 2 or 3 locks, while all others always hold either 3 or 4.
		There are $n$ processes and $3n$ locks in total, hence at all times the global configuration is such that either all locks are taken and the next operation of some process $p$ is $\rel{}$ (and $\get{}$ for all others) or one lock is free and all processes have a $\get{}$ as their next operation.
		
		Now say process $p_n$ has started executing $\send(b_{j+1})$ by releasing $(b_{j+1})_n$. This means some other process must have taken $(b_{j+1})_n$, which can only be $p_{n-1}$. The only possibility is that $p_{n-1}$ then releases $(b_{j+1})_{n-1}$, which can only be taken by $p_{n-2}$, ... We must end up executing $\acqs(b_{j+1})$, which ends with $(b_{j+1})_0$ free, which can only be taken by $p_n$.
		
		By continuing this reasoning we conclude that $\run_{j+1}=\run_j seq(b_{j+1})$, proving the lemma.
	\end{proof}

As all $p_i$ execute $end_i$ in $\run$, in particular $\run|_{p_n}$ ends with $end^n$, hence it is necessarily of the form $\start_n \send(b_1) \cdots \send(b_m) end^n$. 
Let $\run'$ be $\run$ where all $end^i$ have been erased.
The lemma above allows us to conclude that for all $i$, $\run'|_{p_i}$ has $\rec_i(b_1)  \cdots \rec_i(b_m)$ as a suffix. 

Recall that the languages of all $\aut_i$ are included in $11(00+01)^*$.
Moreover, we know that $b_1 \cdots b_m$ is in the language of $\aut_{n}$,
hence $b_1 = b_2 =1$. Furthermore, all $\run'|_{p_i}$ ($i<n$) are of the form $\start_i \rec_i(x_1) \cdots \rec_i(x_r)$ with $x_1 \cdots x_r$ in the language of $\aut_i$.
As the only moment a factor $11$ can appear in a word of those languages is at the beginning, for $\run'|_{p_i}$ to have $\rec_i(b_1) \cdots \rec_i(b_m)$ as a suffix, we must have $\run'|_{p_i} = \start_i \rec_i(b_1) \cdots \rec_i(b_m)$. 

As a consequence, for all $i$ we have $\run|_{p_i} = \start_i \rec_i(b_1) \cdots \rec_i(b_m) end^i$ and thus $b_1 \cdots b_m$ must be accepted by all $\aut_i$.

We have proven that this system had a run in which each $p_i$ reads $end^i$ if and only if there is a word accepted by all $\aut_i$.

As that condition is easily expressible as a "regular objective", we obtain the \PSPACE-hardness of the "regular verification problem" for "sound" "exclusive" "LSS" with 6 locks per process.
However, our goal was to prove the \PSPACE-hardness of the "process deadlock problem" for "sound" "exclusive" "LSS".

To do so, we add a process $q$ and locks $\ell_{i}$ for $1 \leq i \leq n+1$ so that the transition system of $q$ simply takes $\ell_{n}$ and then goes to a state with a self-loop executing $\nop$. We also add, for each $1 \leq i \leq n$, a sequence of transitions from $stop_i$ which take $\ell_i$, then $\ell_{i-1}$ and release $\ell_i$ if $i \geq 2$, and simply take $\ell_i$ if $i=1$, to end up in a state with no outgoing transition.

We show that there is a "process-fair" run with a finite projection on $q$ if and only if there is one in the previous "LSS" such that each $p_i$ executes $end_i$.

If the latter is true, then we just take the same run and prolong it so that each $p_i$ takes $\ell_i$. Then all $\ell_i$ are taken, and all processes need some $\ell_i$ to advance, we have reached a global deadlock (in particular the run is "process-fair", and its projection on $q$ is finite).

Conversely, suppose we have a "process-fair" run in the new "LSS" with a finite projection on $q$. Then $q$ must be blocked, which is only possible if $\ell_n$ is held forever by $p_n$, which in turn is only possible if $\ell_{n-1}$ is held forever by $p_{n-1}$... We conclude that all $p_i$ must be holding $\ell_i$ forever from some point on, and thus that they all read $end_i$.

We project that run to erase all actions getting an $\ell_i$. We obtain a run of the previous system in which every process has executed $end_i$.

As a result, the new "LSS" has a "process-fair" run in which $q$ is blocked if and only if the former "LSS" has a run in which every $p_i$ has executed $end_i$, if and only if the $\aut_i$ recognise a common word.

As a result, the "process deadlock problem" is \PSPACE-complete for "sound" "exclusive" "LSS" with 8 locks per process. 

==> Ptimeproof.tex <==
\section{Proof of Proposition~\ref{prop:ptime-exclusive}}
\label{app:ptime-exclusive}

\PTIMEEXCLUSIVE*


Let $\tss$ be a "sound" "exclusive" "2LSS" and $p$ a process of $\tss$.	

\begin{lemma}\label{lem:fair-exclusive}
	Let $(s_p, B_p)_{p \in \Proc}$ be a "global configuration" and for each process $p$ let $u'_p$ be a local run starting in $(s_p, B_p)$ and such that $u'_p$ is either infinite or leads to a state with no outgoing transitions.
	
	There exists a "process-fair" global run $\run$ from $(s_p, B_p)_{p \in \Proc}$ such that for all $p$ its projection $\run_p$ on $\S_p$ is a prefix of $u'_p$.
\end{lemma}

\begin{proof}
	We construct $\run$ by iterating the following step:
	For each $p$ we set $u'_p = v_p w_p$ with $v_p$ the prefix of $u'_p$ executed so far.
	We select uniformly at random a process $p \in \Proc$. If it can execute the first action of $w_p$ then we let it do so, otherwise we do nothing.
	
	We iterate this procedure indefinitely.
	This produces a (possibly finite) global run of the system such that its local projections are prefixes of the $u'_p$. We prove that it is "process-fair".
	
	Let $p \in \Proc$, assume that $p$ has an available action at infinitely many steps.
	As our "LSS" is "exclusive", whenever $p$ has an available action and is in some state $s$,
	either all outgoing transitions are executing an operation $\nop$ or $\rel{}$ (and thus can all be executed as the system is "sound"), or they all acquire the same lock $t$ (as the system is "exclusive").
	Hence if one outgoing transition can be executed , they all can and thus in particular the next action of $u'_p$ is available.
	As a result, $p$ can execute the next action of $u_p$ at infinitely many steps, and thus will progress infinitely many times in $u_p$.
	
	In conclusion, with this procedure we either reach a "global deadlock", or we always have an available action, implying that at least one process will be able to progress infinitely many times and that the resulting run $u$ is infinite. 
	In the latter case, all processes that can execute an action at infinitely many steps of the run will do so, proving that the run is "process-fair".
\end{proof}

\begin{definition}
	Define the graph $G$ whose vertices are locks and with an edge $t_1 \edge{p} t_2$ if and only if the process $p$ has a local run $\run_p$ ending in a state where all outgoing transitions acquire $t_2$ and such that $\Owns(\run_p) = \set{t_1}$. We say that $\run_p$ ""witnesses"" the edge $t_1 \edge{p} t_2$.
\end{definition}

\begin{lemma}
	\label{lem:always-one-weak}
	For all $p \in \Proc$, if there is a $p$-labelled edge $t_1 \edge{p} t_2$ in $G$  then either $t_1 \edge{p} t_2$ is "witnessed" by a run with a weak pattern or its reverse $t_2 \edge{p} t_1$ is in $G$ and is "witnessed" by a run with a weak pattern.
\end{lemma}

\begin{proof}
	As $p$ has an edge $t_1 \edge{p} t_2$ in $G$, there is a local run which acquires both locks of $p$ at the same time. Let $\run_p$ be such a run of minimal length. The last operation in $\run_p$ must be a $\get{}$, by minimality, hence $\run_p$ is of the form $\run'_p a$ with $op(a) = \get{t}$ for some $t \in \set{t_1, t_2}$.
	Furthermore, suppose the last operation in $\run'_p$ besides $\nop$ is a $\rel{}$, then there is a previous configuration in $\run_p$ in which $p$ holds both of its locks, contradicting the minimality of $\run_p$. Hence $\run'_p$ has a weak pattern, and it leads to a state where $p$ may acquire $t$, thus has to acquire $t$ as the system is "exclusive". Furthermore $p$ is then holding its other lock, therefore $\run'_p$ "witnesses" an edge in $G$.
\end{proof}

\begin{lemma}
	\label{lem:cond-cycle}
	If $p$ has a reachable transition acquiring some lock $t$ and there is a path from $t$ to a cycle in $G$ then there is a "process-fair" global run with a finite projection on $p$. 
\end{lemma}

\begin{proof}
	Let $t = t_0 \edge{p_1} t_1 \edge{p_2} \cdots \edge{p_k} t_k$ be such a path in $G$ and let $t_k = t'_1 \edge{p'_1} \cdots t'_n \edge{p'_n} t'_{n+1} = t'_1 = t_k$ be such  a cycle.
	
	For all $1 \leq i \leq k$ we choose a run $\run_i$ "witnessing" $t_{i-1} \edge{p_i} t_i$. Similarly for all $1 \leq j \leq n$ we choose a run $\run'_j$ "witnessing" $t'_{j} \edge{p'_i} t'_{j+1}$, and we choose it so that it has a weak pattern whenever possible.
	
	\paragraph{Case 1: }If there exists $j$ such that $\run'_j$ has a weak pattern, then we proceed as follows: Let $\run'_j = u_j v_j$ so that $u_j$ is the maximal "neutral" prefix of $\run_j$. We execute $u_j$, leaving all locks free.
	Let $m$ be the maximal index such that $t_m \in \set{t'_1, \cdots, t'_n}$. We execute all $\run_i$ in increasing order for $1 \leq i \leq m$.
	
	Then we execute $\run'_{j+1} \cdots \run'_n \run'_1 \cdots \run'_{j-1}$ and then $v_j$. Then we end up in a configuration where all $p_i$ with $i\leq m$ are holding $t_{i-1}$ and need $t_i$ to advance, while all $p'_i$ are holding $t'_i$ and need $t'_{i+1}$ to advance. As $t_j \in \set{t'_1,\ldots, t'_n}$, all those processes are blocked, and in particular $t = t_0$ is held by a process which will never release it.
	
	As $p$ has a reachable transition taking $t$, we can define $\run_p$ as a shortest run that ends in a state where some outgoing transitions takes a lock of $\set{t_0, \ldots, t_m, t'_1, \ldots, t'_n}$. By minimality this run can  be executed, as all other locks are free. 
	By exclusiveness, it reaches a state where all transitions take the same non-free lock.
	
	By Lemma~\ref{lem:fair-exclusive} we can extend this run into a "process-fair" one, whose projection on $p$ can only be $\run_p$, as $p$ will never be able to advance further.
	
	\paragraph{Case 2: }Now suppose there is no $j$ such that $\run'_j$ has a weak pattern, then as we took all $\run'_j$ with weak patterns whenever possible, it means there is no local run with a weak pattern "witnessing" any of the $t'_j \edge{p'_j} t'_{j+1}$.
	We can then apply Lemma~\ref{lem:always-one-weak} to show that the reverse cycle $t'_1 = t'_{n+1} \edge{p'_n} t'_n \cdots \edge{p'_1} t'_1$ exists in $G$ and all its edges are "witnessed" by runs with weak patterns.
	Hence we can apply the arguments from the previous case using this cycle to conclude.
\end{proof}

\begin{lemma}
	\label{lem:cond-inf}
	If $p$ has a reachable transition acquiring some lock $t$ and there is a path in $G$ from $t$ to some $t'$ such that there is a process $q$ with an infinite local run $\run_q$ acquiring $t'$ and never releasing it (i.e., such that $t' \in \Owns(\run_q)$), then there is a "process-fair" global run with a finite projection on $p$. 
\end{lemma}
\begin{proof}
	Let $t = t_0 \edge{p_1} t_1 \edge{p_2} \cdots \edge{p_{k}} t_k = t'$ be the shortest path from $t$ to $t'$.
	Let $\run_p$ be a local run of $p$ acquiring $t$ at some point, either infinite or leading to a state with no outgoing transition. 
	For each $1 \leq i \leq k$ we select a local run $\run_i$ of $p_i$ "witnessing" $t_{i-1} \edge{p_i} t_i$.
	Furthermore we select those $\run_i$ with "weak patterns" whenever possible. 
	Let $t_q$ be the other lock used by $q$ besides $t'$, and let $\run_q$ be an infinite run of $q$ in which $t'$ is eventually taken and never released.
	We can decompose $\run_q$ as $u_q v_q$ where $u_q$ is the largest "neutral" prefix of $\run_q$. 
	We distinguish several cases:
	
	\paragraph{Case 1:} $t_q \notin \set{t_0, \ldots, t_k}$, or $t_q$ is not used in $v_q$. Then we can execute $u_q$, leaving all locks free, then $\run_1 \cdots \run_k$, which can be done as the execution of $\run_1 \cdots \run_i$ leaves $t_{i}, \ldots, t_k$ free and thus $\run_{i+1}$ can be executed.
	Let $v_q = v'_q v''_q$ with $v'_q$ a prefix of $v_q$ large enough so that $t'$ is held by $q$ and never released later.
	Then as no $t_i$ is used in $v_q$, we can execute $v'_q$. 
	Let $\run$ be the run constructed so far.
	Then by Lemma~\ref{lem:fair-exclusive} we can construct a "process-fair" run $\run'$ starting in the last configuration of $\run$ whose projection on $q$ is a prefix of $v''_q$ (thus $t_k$ is never released and thus neither are $t_0, \ldots, t_{k-1}$) and whose projection on $p$ is a prefix of $\run_p$ (and thus finite as $\run_p$ tries to acquire $t$, which is never free). As a consequence, $\run\run'$ is a "process-fair" run whose projection on $p$ is finite.
	
	\paragraph{Case 2:} $t_q = t_j$ for some $0 \leq j \leq k$ and $\run_q$ acquires $t_j$ at some point and never releases it. Then we apply the same reasoning as in the previous case for the path $t = t_0 \edge{p_1} \cdots \edge{p_j} t_j$.
	
	\paragraph{Case 3:} $t_q = t_j$ for some $0 \leq j \leq k$ and $t_j$ is used in $v_q$ but not kept indefinitely.
	
	\paragraph{Subcase 3.1:} there is an edge $t' \edge{q} t_j$.
	Then we have a path from $t$ to a cycle $t_j \edge{p_{j+1}} \cdots \edge{p_k} t' \edge{q} t_j$.
	Hence by Lemma~\ref{lem:cond-cycle}, there is a "process-fair" global run with a finite projection on $p$. 
	
	\paragraph{Subcase 3.2:} One of the runs $\run_i$ has a "weak pattern" $\dashover{\set{t_{i-1}}}$. 
	We decompose $\run_i$ as $u_i v_i$ with $u_i$ its largest "neutral" prefix.
	Then we execute $u_i$, then $\run_{i+1} \cdots \run_{k}$. After that we execute a prefix $\run'_q$ of $\run_q$ such that at the end $q$ holds only $t'$, and does not release it later. This prefix exists as $q$ never keeps $t_j$ indefinitely in $\run_q$. We decompose $\run_q$ as $\run'_q \run''_q$. Then we execute $\run_1 \cdots \run_{i-1} \run'_i$. All those runs can be executed as before executing each $\run_{i'}$ both locks of $p_{i'}$ are free, and before executing $v_i$, $t_{i-1}$ is free, which is all that is needed to execute $v_i$ as $\run_i$ has a "weak pattern". Let $\run$ be the run constructed so far.
	Then by Lemma~\ref{lem:fair-exclusive} we can construct a "process-fair" run from the configuration reached by $\run$ whose projection on $q$ is a prefix of $\run''_q$ and whose projection on $p$ is a prefix of $\run_p$.
	As a consequence, $t' = t_k$ is never released in $\run''_q$ and thus neither are $t_0, \ldots, t_{k-1}$. As $\run_p$ tries to take $t = t_0$ at some point, its prefix executed in $\run'$ is finite. 
	Hence $\run \run'$ is a "process-fair" run with a finite projection on $p$.
	
	\paragraph{Subcase 3.3:} There is no edge $t' \edge{q} t_j$ and all $\run_i$ have "strong patterns".
	When executing the $v_q$ part of $\run_q$, $q$ holds a lock at all times, and holds $t_j$ at some point and $t'$ at some point, hence it has to have both at the same time at some moment.
	Hence there is a moment at which $q$ holds one of the locks and is about to get the other. As the system is "exclusive", it means all its available transitions take that lock.
	Hence there is an edge  $t' \edge{q} t_j$ or $t_j \edge{q} t'$ in the graph. As we assumed that there is no edge $t' \edge{q} t_j$, there is one $t_j \edge{q} t'$. 
	Furthermore, as we selected the $\run_i$ so that they had weak patterns whenever possible, it means that for all $i$ there is no run with a weak pattern "witnessing" $t_{i-1} \edge{p_i} t_i$.
	By Lemma~\ref{lem:always-one-weak} this means that there are edges $t_k \edge{p_k} t_{k-1} \edge{p_{k-1}} \cdots \edge{p_{j+1}} t_j$. With the edge $t' \edge{q} t_j$, we obtain a cycle in $G$ with a path from $t$ to it.
	By Lemma~\ref{lem:cond-cycle}, there is a "process-fair" global run with a finite projection on $p$. 
	
	This concludes our case distinction, proving the lemma.	
\end{proof}

\begin{lemma}
	\label{lem:cond-stop}
	If $p$ has a reachable transition acquiring some lock $t$ and there is a path in $G$ from $t$ to some $t'$ such that there is a process $q$ with a local run $\run_q$ with $t' \in \Owns(\run_q)$ and going to a state with no outgoing transitions, then there is a "process-fair" global run with a finite projection on $p$. 
\end{lemma}
\begin{proof}
	Let $s_q$ be the state reached by $\run_q$, we add a self-loop on it with a fresh letter $\#$. As there are no other outgoing transitions from $s_q$ this does not break the exclusiveness. It does not change $G$ either.
	Then $\run_q \#^\omega$ is an infinite run acquiring $t'$ and never releasing it.
	
	Hence by Lemma~\ref{lem:cond-inf}, there is a "process-fair" run $\run$ in this new system whose projection on $p$ is finite. Let $h$ be the morphism such that $h(\#) = \epsilon$ and $h(a) = a$ for all other letters $a$. 
	Then $h(\run)$ is a "process-fair" run of the original system: it is a run as $\#$ does not change the configuration, meaning that all actions of $h(\run)$ can be executed. For the same reason, if a process $p'$ other than $q$ only has finitely many actions in $h(\run)$, then the same is true in $\run$, thus there is a point after which no configuration allows $p'$ to move in $\run$, and thus in $h(\run)$ as well. As for $q$, either it only executes $\#$ from some point on, meaning it has reached $s_q$ and will be immobilised in $h(\run)$, or it never executes any $\#$, in which case $h(\run) = \run$ and it follows the same configurations in both.
\end{proof}



\begin{lemma}\label{lem:exclusiveGraph}
	There is a "process-fair" run whose projection on $p$ is finite if and only if there is a local run $\run_p$ of $p$ leading to a state where all outgoing transitions take some lock $t$ and either 
	
	\begin{enumerate}		
		\item\label{Cx1} $p$ has a local run leading to a state with no outgoing transitions.
		
		\item\label{Cx2} or there is a path from $t$ to a cycle in $G$
		
		
		\item\label{Cx3} or there is a path in $G$ from $t$ to some lock $t'$ and there is a process $q$ with a local run $\run_q$ with an 
		"infinitary pattern" with $t' \in \Owns(\run_q)$. 
	
		
		\item\label{Cx4} or there is a path in $G$ from $t$ to some lock $t'$ and there is a process $q$ with a local run $\run_q$ such that $t' \in \Owns(\run_q)$ and leading to a state with no outgoing transitions.
	\end{enumerate}
\end{lemma}

\begin{proof}
	We start with the left-to-right implication: Say there is a run $\run$ whose projection on $p$ is finite. For each process $p' \in \Proc$ let $\run_{p'}$ be its local run. 
	
	Then $\run_p$ has to end in a state where all available transitions acquire a
	lock $t$. If there are no transitions at all, condition~\ref{Cx1} is
	satisfied. If there is at least one such transition, then $t$ is held
	forever by some other process $p_1$.
	
	We construct a path $t = t_0 \edge{p_0} t_1 \edge{p_1} \cdots$ in $G$ so that all $t_i$ are held indefinitely by some process after some point in the run.
	Say we already constructed those up to $i$.
	
	There is a process $p_{i}$ holding $t_i$ indefinitely.
	If $\run_{p_{i}}$ is infinite, then condition~\ref{Cx3} is satisfied. Otherwise, $\run_{p_{i}}$ is finite, and with a "finitary pattern" such that $t_i \in \Owns(\run_{p_i})$.
	
	If this local run ends up in a state with no outgoing transition then condition~\ref{Cx2} is satisfied, otherwise it must have no choice but to acquire some lock $t'_{i+1}$.
	Hence we construct an infinite path
	$t'_0 \edge{p'_0} t'_1 \edge{p'_1} \cdots$ in $G$.
	
	The set of processes is finite, hence there exist 
	$i < j$ such that $t_i = t_j$, meaning we have reached a cycle. Thus condition~\ref{Cx4} is satisfied.
	
	For the other direction, suppose there exists $t$ as in the statement of the lemma, so that one of the conditions is satisfied.
	
	If condition~\ref{Cx1} is satisfied, then we have a finite run $\run_p$ leading to a state with no outgoing transition. We execute it and then prolong it into a global "process-fair" run by choosing a process uniformly at random and executing one of its available actions if there is any (similarly to the proof of \ref{lem:fair-exclusive}). 
	We obtain a "process-fair" run in which $p$ only has finitely many actions. 
	If condition~\ref{Cx2} is satisfied then we have the result by Lemma~\ref{lem:cond-cycle}.
	If condition~\ref{Cx3} is satisfied then we have the result by Lemma~\ref{lem:cond-stop}.
	If condition~\ref{Cx4} is satisfied then we have the result by Lemma~\ref{lem:cond-inf}.
%	Otherwise we proceed in two steps: first ensure that $t'$ is blocked forever with a finite run $\run$ with actions from a subset of processes $P$, and then use a path from $t$ to $t'$ in $G$ containing no process of $P$ to block $t$ as well.
%	
%	We distinguish cases according to which condition is satisfied for the first step, the second step is common to all cases.
%	
%	If condition~\ref{Cx2} is satisfied, we have a finite run $\run_q$ of some process $q$ such that $t' \in \Owns_q(\run_q)$ and leading to a state with no outgoing transition. We set $\run = \run_q$ and $P = \set{q}$.
%	
%	If condition~\ref{Cx3} is satisfied, then we have an infinite local run $\run_q$ such that eventually $q$ never releases $t'$. We execute a prefix of $\run_q$ up to a point where either:
%	\begin{itemize}
%		\item $q$ holds both of its locks and keeps them indefinitely afterwards.
%		
%		\item or $q$ only holds $t'$ and keeps it forever afterwards.    
%	\end{itemize}
%	We set $\run$ to be that prefix and $P = \set{q}$.
%	
%	If condition~\ref{Cx4} is satisfied, then we execute first the largest prefix $\run^p_k$ of $\run_k$ such that $\Owns_{p_k}(\run_k) = \emptyset$. Then we execute  for each $0 \leq i \leq k-1$ in increasing order the local run $\run^{t_i,t_{i+1}}_{p_i}$ of process $p_i$. Finally we can execute the rest of $\run_k$.
%	This is all possible as before we execute all $\run^{t_i,t_{i+1}}_{p_i}$ (with $i \leq k-1$) $t_i$ and $t_{i+1}$ are free. Furthermore as $\run_k$ has a weak pattern $\dashover{\set{t_k}}$, after executing $\run^p_k$ , the remaining actions only take $t_k$ (which is free at that point) and do nothing else on locks. We set $P = \set{p_1, \ldots, p_k}$ and $\run$ as the run described above.
%	
%	In all cases we have a finite run of processes of $P$ leading to a configuration where all locks that are not free will never be released, and $t'$ is one of them. Let $\Theta$ be the set of non-free locks after executing $\run$.
%	
%	Then let $t = t'_0 \edge{p'_0} \cdots \edge{p'_{n-1}} t'_n$ be a path in $G$ of minimal length from $t$ to some $t_n \in \Theta$. It exists as there is a path from $t$ to $t' \in \Theta$ in $G$.  All locks are free at the start, hence we can execute (in increasing order) for each $i$ the local run $\run_{p'_i}^{t'_i, t'_{i+1}}$. As we took a shortest path, no $t'_i$ is in $\Theta$.
%	
%	After we do that, we execute $t'$ 
\end{proof}


	To conclude the proof of Proposition~\ref{prop:ptime-exclusive}, by Lemma~\ref{lem:exclusiveGraph}, we only have to check the four conditions listed in its statement.	
	Here is our algorithm: 
	
	We start by looking, in the transition system of process $p$, for a reachable local state with no outgoing transition. If there is one, we accept.

	Then we compute all pairs $(q, t)$ such that either there is an infinite run of process $q$ keeping $t$ indefinitely from some point on or there is a run $\run_q$ with $t \in \Owns(\run_q)$ leading to a state with no outgoing transitions. 
	As our system is "sound", the set of locks a process has is determined by its state. Let $\ownfunc_p$ be the function described in Definition~\ref{def:soundness}.
	Then we compute all pairs $(t, t')$ such that some process $p'$ has a reachable state $s$ with $\ownfunc_{p'}(s) = \set{t}$ and all outgoing transitions of $s$ acquiring $t'$.
	We obtain the edges of $G$.
	
	For both locks of $p'$, we check that there is a reachable transition acquiring it, and there is a path in $G$ to either a cycle or to a $t$ from one of the pairs $(q,t)$ computed above. If it is the case for one of them, we accept, otherwise we reject.
	This can all be done in polynomial time, proving the proposition.

==> lower.tex <==
\section{Lower bounds}\label{sec:lower}

In this section we sketch the two remaining lower bounds, namely
\EXPTIME-hardness for "nested" locks and undecidability for arbitrary
locks.
The full proofs are in the appendix.

\begin{restatable}{proposition}{PropExpHard}
	\label{prop:EXPTIME-hard}
	The "DLSS verification problem" for "nested" "DLSS" and
        Büchi objective is \EXPTIME-hard.
        The result holds even if the Büchi objective refers to a
        single process.
\end{restatable}

\begin{proof}[Proof sketch]
	We show that the difficulty of the problem stems from the
        systems and not the specification, by proving that checking if
        some copy of a particular process has an infinite run is already
        \EXPTIME-hard. 
	
	For this we provide a reduction from the emptiness problem for the
        % \ancain{if we reduce from the intersection problem for Buechi
        %   TA over infinite trees, we may simplify by eliminating $z,z1,z2$}
        intersection of top-down tree automata over finite trees.
        
        The  "DLSS" creates one process for each node of
        the tree $T$ that should belong to the intersection.
        Each such process guesses the states of the parent node, and
        spawns some processes in charge of checking the guesses.
        The checks are done by taking forever suitable locks.
        Process-fairness ensures that if some guess was wrong, then a
        certain lock $\ell_t$  is taken in such a way that the particular
        process does not satisfy its Büchi condition.

        In more detail, each node of $T$ is represented by a copy of
        process $p_a^i$ 
        or  $p_b^i$, depending on the letter $a$ or $b$ its parent is
        labeled with, and on whether it is a left or right child of
        its parent ($i=0$ and $i=1$, respectively).
           Process $p_a^1$ proceeds as follows: it chooses for each of
        its children a letter and spawns the corresponding processes,
        sharing some of the variables that are needed by the children
        to check its own state.
        If the node represented by $p_a^1$ is a leaf, then $p_a^1$
        spans a unique child $p_c$.
        For each $1 \leq i \leq k$, process $p_a^1$ then guesses the
        state $s$ of its parent in $\aut_i$ and spawns a process $\ch$
        in charge of checking the guess, so whether the lock
        associated with $x_i^s$ is  taken.
        If that lock is not taken, then process $\ch$ can ultimately
        take it due to process-fairness, and then it also takes lock
        $\ell_t$, preventing the satisfaction of the acceptance
        condition. 
	
	
	The final problem is that  the construction may  end up producing 
        infinitely many nodes for $T$.
        By using additional locks that need to be taken bottom-up, we
        guarantee that $T$ is finite.
\end{proof}




\medskip

We conclude with the sketch of proof for Theorem~\ref{th:undec}.


% \begin{theorem}\label{th:undec}
%   It is undecidable to know if a "DLSS" satisfies a
%   reachability condition.
%   The result holds even if the "DLSS" is finite-state and  every
%   process uses at most 4 locks. 
% \end{theorem}

\begin{proof}[Sketch of proof for Theorem~\ref{th:undec}]
  
The proof idea is to simulate an accepting run of TM $M$ using $n$ cells by
spawning a chain of $n$ processes, $P_0,\dots,P_{n-1}$.
We assume that $M$ accepts when the head is leftmost, and use a
reachability condition for the initial process.

The initial process $P_0$ uses three locks, called $a,b,c_1$, and acquires
$a,b$ before spawning $P_1$.
Process $P_1$ uses locks $a,b,c_1$, plus a fresh lock $c_2$.
It acquires $c_1$ before spawning $P_2$.
More generally, process $P_k$ ($1\le k <n-1$) uses locks
$a,b,c_k,c_{k+1}$, and it acquires $c_k$ before spawning the next
process $P_{k+1}$.
The last process $P_{n-1}$ uses only three locks, $a,b,c_{n-1}$.

A configuration $(p,k,A_0 \dots A_{n-1})$ of the TM corresponds to
each $P_j$ storing $A_j$, with process $P_k$ storing in addition state
$p$.
The process that corresponds to the head position is the one that
holds the locks $a$ and $b$.
Sending the current state to the suitable neighbor is mimicked by a
sequence of $\get{}$ and $\rel{}$ operations that needs to match a
sequence executed by the neighbor.
If the neighbor does not execute the sequence, or if other processes
get involved during the ``communication'', then the system deadlocks.

\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "m"
%%% End:

